Self-Verification Improves Few-Shot Clinical Information Extraction

Extracting patient information from unstructured text is a critical task in health decision-support and clinical research. Large language models (LLMs) have shown the potential to accelerate clinical curation via few-shot in-context learning, in contrast to supervised learning which requires much more costly human annotations. However, despite drastic advances in modern LLMs such as GPT-4, they still struggle with issues regarding accuracy and interpretability, especially in mission-critical domains such as health. Here, we explore a general mitigation framework using self-verification, which leverages the LLM to provide provenance for its own extraction and check its own outputs. This is made possible by the asymmetry between verification and generation, where the latter is often much easier than the former. Experimental results show that our method consistently improves accuracy for various LLMs in standard clinical information extraction tasks. Additionally, self-verification yields interpretations in the form of a short text span corresponding to each output, which makes it very efficient for human experts to audit the results, paving the way towards trustworthy extraction of clinical information in resource-constrained scenarios. To facilitate future research in this direction, we release our code and prompts.

==> tabs/f1_full.tex <==
\begin{tabular}{llll}
\toprule
& ChatGPT & GPT-4 & GPT-3.5 \\
\midrule
Clinical trial arm, original & 0.342\err{0.010} & 0.419\err{0.008} & 0.512\err{0.009} \\
Clinical trial arm, self-verified & 0.456\err{0.007} & 0.530\err{0.010} & 0.575\err{0.003} \\
Medication name, original & 0.892\err{0.004} & 0.884\err{0.003} & 0.929\err{0.002} \\
Medication name, self-verified & 0.898\err{0.002} & 0.910\err{0.001} & 0.935\err{0.001} \\
Medication status, original & 0.194\err{0.010} & 0.139\err{0.011} & 0.561\err{0.058} \\
Medication status, self-verified & 0.346\err{0.025} & 0.456\err{0.048} & 0.581\err{0.062} \\
MIMIC-III ICD9, original &  & 0.65\err{0.02} & \\
MIMIC-III ICD9, self-verified &  & 0.68\err{0.007} & \\
MIMIC-IV ICD9, original &  & 0.72\err{0.03} & \\
MIMIC-IV ICD9, self-verified &  & 0.75\err{0.004} & \\
MIMIC-IV ICD10, original &  & 0.49\err{0.02} & \\
MIMIC-IV ICD10, self-verified &  & 0.53\err{0.002} & \\
\bottomrule
\end{tabular}
